Constraining the coherence scale of the interstellar magnetic field using TeV gamma-ray observations of supernova remnants

Galactic cosmic rays (CRs) are believed to be accelerated at supernova remnant (SNR) shocks. In the hadronic scenario the TeV gamma-ray emission from SNRs originates from decaying pions that are produced in collisions of the interstellar gas and CRs. Using CR-magnetohydrodynamic simulations, we show that magnetic obliquity-dependent shock acceleration is able to reproduce the observed TeV gamma-ray morphology of SNRs such as Vela Jr. and SN1006 solely by varying the magnetic morphology. This implies that gamma-ray bright regions result from quasi-parallel shocks (i.e., when the shock propagates at a narrow angle to the upstream magnetic field), which are known to efficiently accelerate CR protons, and that gamma-ray dark regions point to quasi-perpendicular shock configurations. Comparison of the simulated gamma-ray morphology to observations allows us to constrain the magnetic coherence scale $\lambda_B$ around Vela Jr. and SN1006 to $\lambda_B \simeq 13_{-4.3}^{+13}$ pc and $\lambda_B >200_{-10}^{+80}$ pc, respectively, where the ambient magnetic field of SN1006 is consistent with being largely homogeneous. We find consistent pure hadronic and mixed hadronic-leptonic models that both reproduce the multi-frequency spectra from the radio to TeV gamma rays and match the observed gamma-ray morphology. Finally, to capture the propagation of a SNR shock in a clumpy interstellar medium, we study the interaction of a shock with a dense cloud with numerical simulations and analytics. We construct an analytical gamma-ray model for a core collapse SNR propagating through a structured interstellar medium, and show that the gamma-ray luminosity is only biased by 30% for realistic parameters.

==> Makefile <==
# Makefile to produce the article.
PDFLATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: pdflatex
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
DVIPS  =  dvips
FIGURES = 

.PRECIOUS: $(FIGURES)

default: ms.pdf

%.pdf :  $(FIGURES) %.tex
	$(PDFLATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	make clean

%.ps :  $(FIGURES) %.tex
	$(LATEX) $*.tex
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(LATEX) $*.tex
	$(DVIPS) -o $*.ps $*.dvi
	ps2pdf $*.ps
	make clean

figures/%.eps: figures/%_raw.eps figures/%.tex
	(cd figures; latex $*.tex; \
	dvips -E -o $*.eps $*.dvi; \
	perl -ane '{ s/%%BoundingBox: [-0-9]+/%%BoundingBox: 135/g; print}' $*.eps > tmp.eps; \
	mv tmp.eps $*.eps; \
	rm -f *.dvi *.log *.aux)

clean:
	rm -f *.log *.toc *.aux *.dvi *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.dvi *.obj *.bak *.bbl *.blg *.brf \
              ms.pdf *.ps */*.ps *~ */*~ *.bak */*.bak 









